All Languages Matter: Understanding and Mitigating Language Bias in Multilingual RAG

Multilingual Retrieval-Augmented Generation (mRAG) leverages cross-lingual evidence to ground Large Language Models (LLMs) in global knowledge. However, we show that current mRAG systems suffer from a language bias during reranking, systematically favoring English and the query's native language. By introducing an estimated oracle evidence analysis, we quantify a substantial performance gap between existing rerankers and the achievable upper bound. Further analysis reveals a critical distributional mismatch: while optimal predictions require evidence scattered across multiple languages, current systems systematically suppress such ``answer-critical'' documents, thereby limiting downstream generation performance. To bridge this gap, we propose \textit{\textbf{L}anguage-\textbf{A}gnostic \textbf{U}tility-driven \textbf{R}eranker \textbf{A}lignment (LAURA)}, which aligns multilingual evidence ranking with downstream generative utility. Experiments across diverse languages and generation models show that LAURA effectively mitigates language bias and consistently improves mRAG performance.

==> acl-style-files-master/tables/pearson_all.tex <==
\begin{table}[t]
\centering
\small
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|cc|cc}
\toprule
& \multicolumn{2}{c|}{\textbf{MKQA}} & \multicolumn{2}{c}{\textbf{XOR TyDi QA}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\textbf{Setting}
& \textbf{Pearson $r$} & \textbf{$p$-value}& \textbf{Pearson $r$} & \textbf{$p$-value}\\
\midrule
\multicolumn{5}{c}{\textbf{\textit{Command-R-35B}}} \\
\midrule
 BGE-Reranker   &0.198  & $<10^{-100}$ & 0.234  & $2.9\times10^{-40}$ \\ 
\quad\textbf{+ LAURA} &0.237  & $<10^{-100}$ & 0.174  & $1.3\times10^{-22}$ \\ 
Qwen-Reranker&0.158 & $<10^{-100}$ & 0.114 & $1.7\times10^{-10}$ \\ 
\quad\textbf{+ LAURA} & \textbf{0.287}  & $<10^{-100}$ & \textbf{0.304}  & $7.1\times10^{-68}$ \\ 

\midrule
\multicolumn{5}{c}{\textbf{\textit{Llama3-8B-Instruct}}} \\
\midrule
 BGE-Reranker   &0.198  & $<10^{-100}$ & 0.264  & $2.9\times10^{-40}$ \\ 
\quad\textbf{+ LAURA} &0.236  & $<10^{-100}$ & 0.184  & $3.5\times10^{-25}$ \\ 
Qwen-Reranker&0.157 & $<10^{-100}$ & 0.126 & $1.4\times10^{-13}$ \\ 
\quad\textbf{+ LAURA} & \textbf{0.274}  & $<10^{-100}$ & \textbf{0.327}  & $4.2\times10^{-79}$ \\ 

\midrule
\multicolumn{5}{c}{\textbf{\textit{Qwen2.5-7B-Instruct}}} \\
\midrule
BGE-Reranker   &0.188  & $<10^{-100}$ & 0.250  & $1.0\times10^{-45}$ \\ 
\quad\textbf{+ LAURA} &0.247  & $<10^{-100}$ & 0.192  & $1.9\times10^{-27}$ \\ 
Qwen-Reranker&0.161 & $<10^{-100}$ & 0.132 & $1.4\times10^{-12}$ \\ 
\quad\textbf{+ LAURA} &\textbf{0.292}  & $<10^{-100}$ & \textbf{0.311}  & $2.8\times10^{-71}$ \\ 

\bottomrule
\end{tabular}
}
\caption{Pearson correlation between reranker relevance scores (mean of top-5) and downstream answer performance (Recall@3-gram) on MKQA and XOR TyDi QA.}

\label{tab:rerank_corr_all}
\end{table}


==> section/method.tex <==
\section{Language-Agnostic Utility-driven Reranker Alignment}
In this section, we aim to mitigate language bias in multilingual rerankers. Such bias leads models to disproportionately favor documents in English or the query language, even when higher quality evidence exists in other languages. We hypothesize that skewed training data, in which high quality query and document annotations are scarce for low resource languages, is a key factor driving this disparity.

To address this issue, we propose a \textit{language agnostic utility driven reranker alignment} framework (LAURA). This framework reduces language bias by grounding reranker supervision in answer utility instead of relying on language dependent relevance signals. Instead of defining positives based on lexical overlap or language matching, LAURA selects documents according to their contribution to downstream answer quality, thereby reducing reliance on language specific surface features. Specifically, LAURA uses a two stage data construction pipeline (Figure~\ref{fig:data_pipeline}) to generate language agnostic supervision signals, followed by listwise reranker fine tuning. This design promotes balanced cross lingual supervision and aligns reranker preferences with answer correctness, thereby mitigating the over preference for high resource languages.

\subsection{Answer Utility-driven Data Construction}
 % for Language Bias Mitigation
Although many RAG QA datasets are publicly available, most only provide annotations for the correctness of the final answer, without explicit query-document relevance labels. This absence leads to language bias in reranker training. We aim to automatically generate such annotations while maintaining balanced multilingual coverage.

Given a query $q$, we retrieve a candidate document set $D$ from a multilingual corpus. Our objective is to select a positive subset $D_{\text{pos}} \subset D$ consisting of documents that genuinely support answering the query, free from language-specific bias. We use the average answer quality produced by multiple generators conditioned on a document as a proxy for its answer utility.

\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{acl-style-files-master/fig/data_pipeline_full.pdf}
    \vspace{-5pt}
    \caption{Two-stage data construction pipeline in the LAURA framework.}
    \vspace{-5pt}
    \label{fig:data_pipeline}
\end{figure*}

\paragraph{Stage 1: Language-Debiased Subset Selection.}
Directly estimating answer utility on top-ranked retrieved documents can amplify the inherent language bias of multilingual rerankers, which often favor documents in high-resource or query-matched languages. To mitigate this effect, we propose a candidate debiasing stage that filters the candidate set before utility estimation while preserving overall utility.

Given a retrieved document set $D$, we partition documents into disjoint subsets according to their language and apply the same reranker to rank documents \emph{within each subset independently}. From each subset, we retain up to five top-ranked documents as utility candidates. This procedure does not assume language-specific relevance. Instead, it enforces equal exposure across linguistic subsets, preventing the candidate pool from being dominated by documents favored due to language priors rather than informational content.

The retained documents are then evaluated by multiple generators to estimate their average answer quality. Documents achieving the highest generation utility are selected for subsequent supervision construction. In cases where multiple subsets yield identical maximal utility (e.g., all generators produce correct answers), all corresponding documents are preserved. The resulting candidate set is denoted as $D_{\text{balanced}}$.

By decoupling candidate selection from global reranker scores and restricting comparisons to within each subset, this stage reduces language-induced ranking bias while retaining documents that are useful for downstream answer generation.

\paragraph{Stage 2: Document-Level Utility Estimation.}
While Stage~1 ensures cross-lingual coverage, documents in $D_{\text{balanced}}$ may still vary in their actual usefulness. We therefore perform fine-grained document-level utility estimation by evaluating each document independently via generation.

To avoid introducing an implicit language bias through relative ranking alone, we apply an absolute utility threshold $\theta$ and retain only documents whose average generation performance exceeds this threshold. The final positive set $D_{\text{pos}}$ thus consists of documents that demonstrably contribute to answer correctness, independent of language.

Overall, this two-stage procedure yields high-quality, language-debiased training data that grounds reranker supervision in answer utility rather than language preference.

\subsection{Listwise Reranker Fine-Tuning}

Using the constructed training data, we fine-tune the reranker with a listwise learning objective. Given a query $q$ and a candidate set $D$, documents not selected into $D_{\text{pos}}$ are treated as negatives, forming $D_{\text{neg}}$. 

During training, we construct training instances consisting of one positive document and $k$ negative documents, i.e., $(q, d_{\text{pos}}, \{d_{\text{neg}}^{(i)}\}_{i=1}^{k})$, where $d_{\text{pos}} \in D_{\text{pos}}$ and $d_{\text{neg}}^{(i)} \in D_{\text{neg}}$. The reranker produces a relevance score $s(q, d)$ for each document $d \in \mathcal{D}_q$. Training encourages the model to assign the highest score to the positive document within the list. We adopt a softmax cross-entropy loss:
\begin{equation}
\mathcal{L}
= - s(q, d_{\text{pos}})
+ \log \sum_{d \in \mathcal{D}_q} \exp \bigl(s(q, d)\bigr)
\end{equation}

For encoder-only rerankers, $s(q, d)$ is produced directly as a scalar logit. For LLM-based rerankers, the score is derived from the relative logits of predefined
\texttt{positive\_token} and \texttt{negative\_token}, which represent the model’s
preference over relevance labels.
\subsection{Experimental Setups}
\paragraph{LAURA Dataset.} We use data from the MKQA benchmark, selecting only samples that are disjoint from the evaluation test set to avoid data leakage. 

In stage 1, for each question, we retrieve the top-100 candidate documents from a multilingual Wikipedia corpus using the BGE-M3 retriever. 
Within each language group, we apply the multilingual BGE reranker to select the top-5 documents, yielding a language-debiased candidate set. 

During evaluation, we prompt multiple generation models to answer the question conditioned on each document independently and measure answer quality using character-level 3-gram recall. To reduce model-specific bias, we compute each document’s utility score as the average generation performance across a diverse set of four generation models, including Qwen2.5-7B-Instruct, Qwen2.5-14B-Instruct, Llama3-8B-Instruct, and DeepSeek-R1-Distill-Qwen-7B~\citep{deepseekai2025deepseekr1incentivizingreasoningcapability}. The threshold $\theta$ is set to 0.8, ensuring that the documents retain high utility. 

Finally, we construct a total of \textbf{18,360} query--positive documents pairs. Among them, \textbf{1,000} are randomly sampled as the dev set. Detailed statistics of the constructed fine-tuning dataset are reported in Appendix~\ref{sec:stat-of-finetuning-dataset}.

\paragraph{Evaluation Metric.}
To evaluate the effectiveness of LAURA, we adopt Precision@k and NDCG@k to assess the rerank performance on positive documents in the dev set. In addition, we use the PEER~\citep{peer} metric to measure whether the reranker exhibits language-specific bias. PEER is based on the assumption that documents with equal relevance should have similar average rankings across different languages. Higher PEER scores indicate weaker language preference. The detailed definitions of the evaluation metrics are provided in Appendix~\ref{sec:metric_details}.

\paragraph{Training Details.}
We fine-tune BGE-Reranker-V2-M3 using the implementation provided by FlagEmbedding\footnote{\url{https://github.com/FlagOpen/FlagEmbedding}}, and Qwen3-Reranker-0.6B using SWIFT~\citep{swift}. 
For each query, BGE is trained with 1 negative document,
whereas Qwen uses 7 negative documents,
reflecting the stronger capacity of the LLM-based reranker to handle larger candidate lists.
Both models are optimized with AdamW~\citep{adamw}, using a learning rate of $6\times10^{-6}$, and are trained for five epochs.

\subsection{Results of LAURA}

\input{acl-style-files-master/tables/dev_res}

\paragraph{LAURA improves multilingual rerankers' ability to identify relevant documents.}
To evaluate whether rerankers can better identify positive candidates under the LAURA, we assess Precision, NDCG on the dev set before and after training. These metrics directly reflect the rerankers' ability to rank relevant candidates higher.
As shown in Table~\ref{tab:dev_result}, both BGE and Qwen rerankers exhibit consistent improvements after being trained within the LAURA. In particular, Precision@5 increases by approximately 6 points, while NDCG@5 improves by around 13 points across both model families, indicating a stronger capability to place positive candidates at higher ranks.

\paragraph{LAURA improves multilingual rerankers' language fairness.}
We observe that LAURA leads to consistent improvements in language fairness. Beyond the quantitative gains on the dev set measured by the PEER metric, we analyze the language distribution of reranker outputs on the MKQA test set after LAURA training. As shown in Table~\ref{tab:distance_table}, the JS divergence and KL divergence between the post-training distribution and the estimated oracle evidence distribution are substantially reduced, demonstrating that the learned distribution moves closer to the desired target distribution. Moreover, we observe a consistent decrease in the proportion of documents written in English and the query language, suggesting that LAURA mitigates the over-preference for dominant languages and encourages a more balanced multilingual ranking behavior. This indicates that LAURA effectively reduces the original language skew of rerankers. In terms of PEER, LAURA yields an about +7 points for the BGE reranker and about +0.5 points for the Qwen reranker, suggesting that the method systematically mitigates language biases and promotes more equitable performance across languages.


\begin{table}
    \centering
    \resizebox{0.4\textwidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    \textbf{Setting}& \textbf{JS} & \textbf{KL} &\textbf{Entropy}  \\
    \midrule
      BGE-Reranker &0.203&0.186& 2.03 \\ 
    \quad\textbf{+ LAURA}  &\textbf{0.090}&\textbf{0.041} & \textbf{2.27} \\ 
    \midrule
    Qwen-Reranker &0.141&0.122&2.13  \\ 
    \quad\textbf{+ LAURA}  &\textbf{0.129}&\textbf{0.094} & \textbf{2.14}  \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{Language distributional metrics before and after LAURA training on the MKQA test set. JS and KL denote the average distances between vanilla distribution and the estimated oracle distribution. Entropy indicates the average entropy of the vanilla distribution of each query language.}
    \vspace{-10pt}
    \label{tab:distance_table}
\end{table}

\paragraph{LAURA improves downstream generation performance and ranking utility.}
LAURA is designed to enhance reranking quality and improve the alignment between reranking scores and downstream generation. To investigate to what extent the improved reranking capability learned under the LAURA transfers to downstream generation performance, we conduct experiments on the MKQA test set using the setup in Section~\ref{sec:Experimental-Setups}. The results are reported in Table~\ref{tab:qa_res_train}. On the 3-gram recall metric, incorporating LAURA leads to an average improvement of 1.95 points for the Qwen reranker and 1.0 points for the BGE reranker. These results indicate that improving the rerankers' ability to select higher-quality candidates can translate into better downstream generate quality.

To quantitatively assess the change in the relationship between ranking quality and generation performance, we compute the Pearson correlation between the average reranking score of the top-5 documents and the corresponding 3-gram recall scores. After training with LAURA, the Pearson correlation increases by approximately 25\% for the BGE reranker and by about 108\% for the Qwen reranker. This demonstrates that LAURA substantially strengthens the correlation between reranking scores and generation performance, thereby improving the practical utility of the reranking scores for downstream generation.

\input{acl-style-files-master/tables/qa_res_train}


\begin{table}
    \centering
    \small
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}[-0.8ex]{\textbf{Setting}} & \multicolumn{2}{c}{\textbf{Llama}} & \multicolumn{2}{c}{\textbf{Qwen}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
     & \textbf{3-gram} & \textbf{Pearson}& \textbf{3-gram} & \textbf{Pearson} \\
    \midrule
        BGE-Reranker  &  48.9 &0.198 & 46.7 &0.188 \\
        Self-Training  &  48.9 &0.188 & 46.7 &0.202 \\
        mMARCO & 48.7 & 0.132 & 46.3 & 0.137 \\
        LAURA & \textbf{49.9} &\textbf{0.236} & \textbf{47.7} & \textbf{0.247}\\ 
    \bottomrule
    \end{tabular}
    }
    \caption{Performance comparison of LAURA against alternative fine-tuning strategies, including Self-Training (naive supervision using top-5 retrieved candidates) and mMARCO fine-tuning (general-purpose multilingual ranking data).}
    \label{tab:blank_baseline}
\end{table}

\subsection{Comparison Against Fine-tuning Baselines}

We provide additional analysis on two alternative fine-tuning strategies to further validate the effectiveness of LAURA's data construction pipeline.

\paragraph{Self-Training Baseline.}

The first baseline fine-tunes the reranker solely on its own top-ranked outputs as pseudo-positive supervision, directly treating the top-5 re-ranked documents as relevant and all remaining candidates as non-relevant, without any additional filtering or refinement. This setting corresponds to the starting point of LAURA's data construction pipeline and serves as an \textit{empty control} to verify whether LAURA's additional filtering and refinement steps contribute beyond naive supervision. Under this paradigm, the model's existing ranking preferences may be progressively reinforced, as no mechanism is introduced to correct noisy or biased pseudo labels.

\paragraph{Fine-tuning on mMARCO.}

The second baseline fine-tunes the reranker using mMARCO \cite{mmarco}, a widely-used multilingual dataset, to examine whether general-purpose training data can address the specific distribution imbalance in mRAG. We randomly sample 20k queries from mMARCO for training, comparable to the 17,360 queries used by LAURA, ensuring a fair comparison in terms of training scale.

For both baselines, we use the same hyperparameters as in our main experiments. In addition, we ensure that LAURA and the Self-Training baseline are trained on the exact same set of queries, isolating the effect of the data construction strategy rather than the training queries themselves.

As shown in Table~\ref{tab:blank_baseline}, LAURA consistently outperforms both baselines across all settings. The Self-Training baseline fails to surpass BGE-Reranker on certain metrics, indicating that naive pseudo-label supervision can reinforce existing biases rather than correct them. The mMARCO baseline also leads to a slight performance drop compared to BGE-Reranker, suggesting that general relevance signals cannot resolve the specific distribution imbalance in mRAG. These results collectively demonstrate that LAURA's filtering and refinement steps are essential for effective reranker adaptation in mRAG settings.

==> section/related_work.tex <==
\section{Related Work}
mRAG is pivotal for bridging global information gaps and ensuring equitable knowledge access across linguistic barriers. To advance this capability, the community has established a robust foundation spanning diverse benchmarks~\citep{asai-etal-2021-xor, 10.5555/3540261.3540839, liu-etal-2025-xrag} and retrieval architectures~\citep{gao-etal-2022-retrieval, 10.1145/3613447, chirkova-etal-2024-retrieval}.

% \noindent \textbf{Bias Indentification}
Previous studies have conducted preliminary analyses of language preference phenomena in mRAG systems. For instance, \citet{amiraz-etal-2025-cross} investigates multilingual retrieval biases over Arabic–English corpora. \citet{park-lee-2025-investigating} evaluate language bias in multilingual RAG by measuring retrieval ranking shifts.
% Recent studies have identified systematic language biases in these systems, observing a tendency for retrievers and rerankers to favor documents in the query language or high-resource languages like English~\citep{park-lee-2025-investigating, amiraz-etal-2025-cross, qi-etal-2025-consistency}. 
% These biases often limit the utilization of informative evidence from low-resource or linguistically distant languages~\citep{wu2024limitscrosslingualdensepassage, sharma-etal-2025-faux}. 
In comparison, our work moves beyond merely characterizing these preferences to systematically quantify the substantial performance gap resulting from this linguistic misalignment.

To mitigate these biases, prior research has largely relied on translation-centric strategies, such as mapping queries or documents to a shared pivot language~\citep{moon-etal-2025-quality, amiraz-etal-2025-cross, park-lee-2025-investigating}. However, these pipeline-level heuristics depend heavily on the capability of translation models and do not fundamentally correct the ranking objective. 
In comparison, we propose to align rerankers directly with generation utility, training the model to prioritize answer-critical evidence regardless of the source language.

==> tables/dev_res.tex <==
\begin{table}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{lccccc}
        \toprule
        \multirow{2}{*}[-0.8ex]{\textbf{Setting}} & \multicolumn{2}{c}{\textbf{Precision}} & \multicolumn{2}{c}{\textbf{NDCG}}& \multirow{2}{*}[-0.8ex]{\textbf{PEER}}  \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
         & \textbf{@5} & \textbf{@10} & \textbf{@5} & \textbf{@10} &  \\ 
        \midrule
        BGE-Reranker & 0.3400 & 0.2712 & 0.4666 & 0.4904& 0.5941 \\ 
        \quad\textbf{+ LAURA}  & \textbf{0.3830} & \textbf{0.3149} & \textbf{0.5531} & \textbf{0.5925}&\textbf{0.6627} \\ 
        \midrule
        Qwen-Reranker & 0.2702 & 0.2206 & 0.3695 & 0.3921&0.6606 \\ 
        \quad\textbf{+ LAURA}  & \textbf{0.3546} & \textbf{0.2847} & \textbf{0.5214} & \textbf{0.5496}&\textbf{0.6720} \\ 
        \bottomrule
    \end{tabular}}
    \caption{Reranking results of BGE-Reranker-V2-M3 (BGE-Reranker) and Qwen3-Reranker-0.6B (Qwen-Reranker) on the dev set before and after LAURA training. PEER measures language bias in the reranker, with higher values indicating weaker language preference.}
    \vspace{-15pt}
\label{tab:dev_result}
\end{table}

==> tables/main_results.tex <==
\begin{table*}[t]
\centering
% \small
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccccccccccc|c}
\toprule
\textbf{Setting}
& ar & de & en & es & fi & fr & it & ja & ko & pt & ru & th & zh & \textbf{Avg.} \\

\midrule
\multicolumn{15}{c}{\textbf{\textit{Llama3-8B-Instruct}}} \\
\midrule

Upper-limit& 53.6 & 76.5 & 79.3 & 76.8 & 73.4 & 76.7 & 77.0 & 47.9 & 41.0 & 78.4 & 68.0 & 44.1 & 33.8 & 63.6 \\
BGE-Reranker   & 32.7  & 62.8  & 70.1  & 63.0  & 58.1  & 64.4  & 63.9  & 29.2  & 25.5  & 66.4  & 51.9  & 26.4  & 21.7  & 48.9   \\
\quad\textbf{+ LAURA} & 33.2  & 64.8  & 69.8  & 65.7  & 59.9  & 66.7  & 65.5  & 28.9  & 24.9  & 69.1  & 50.8  & 26.9  & 22.2  & \textbf{49.9}  \\
Qwen-Reranker& 28.9 & 60.9  & 67.8 & 62.7 & 54.2 & 63.7 & 62.2 & 28.2 & 23.3 & 66.3 & 47.4 & 24.8 & 21.9 & 47.1 \\ 
\quad\textbf{+ LAURA} & 31.6  & 63.3  & 70.1  & 65.5  & 57.3  & 66.1  & 65.0  & 28.2  & 23.8  & 68.4  & 50.5  & 26.7  & 22.7  & 49.2  \\ 
\midrule
\multicolumn{15}{c}{\textbf{\textit{Qwen2.5-7B-Instruct}}} \\
\midrule

Upper-limit & 51.4 & 73.7 & 76.2 & 75.6 & 71.5 & 71.6 & 73.8 & 44.9 & 38.9 & 73.8 & 63.1 & 39.0 & 42.8 & 61.3 \\
BGE-Reranker   & 33.8  & 59.6  & 65.4  & 62.3  & 55.5  & 56.6  & 60.2  & 28.0  & 26.5  & 60.5  & 45.7  & 23.5  & 29.0  & 46.7  \\ 
\quad\textbf{+ LAURA} & 33.9  & 61.0  & 66.0  & 64.2  & 58.4  & 58.8  & 61.8  & 29.4  & 25.7  & 63.4  & 44.8  & 23.4  & 29.5  & \textbf{47.7} \\
Qwen-Reranker & 31.4 & 58.0  & 63.3 & 61.3 & 52.8 & 54.4 & 57.9 & 27.2 & 24.7 & 59.3 & 42.3 & 22.3 & 28.7 & 44.9\\ 
\quad\textbf{+ LAURA} & 33.1  & 59.2  & 65.2  & 63.9  & 55.3  & 57.8  & 61.9  & 28.1  & 25.0  & 62.6  & 44.1  & 22.7  & 28.7  & 46.7 \\ 
\bottomrule
\end{tabular}
}
\vspace{-3pt}
\caption{Performance comparison between the vanilla document reranking and the oracle evidence estimation settings on MKQA.
All results are reported using character 3-gram recall. \textbf{Bolded results} denote the best performance among all non–upper-limit settings.}
\label{tab:mkqa_xor_upper}
\end{table*}



==> tables/pearson.tex <==
\begin{table}[t]
\centering
\small
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{1.2}
\resizebox{0.48\textwidth}{!}{
% \begin{tabular}{l l c c}
\begin{tabular}{llcc}
\toprule
\textbf{Reranker} & \textbf{Model} & \textbf{Pearson} & \textbf{p-value} \\
\midrule
\multirow{2}{*}{BGE-Reranker}
 & Llama3-8B-Instruct & 0.188 & $3.8 \times 10^{-290}$ \\
 & Qwen2.5-7B-Instruct & 0.198  & $1.0 \times 10^{-320}$ \\
\midrule
\multirow{2}{*}{Qwen-Reranker}
 & Llama3-8B-Instruct & 0.129 & $1.2 \times 10^{-135}$ \\
 & Qwen2.5-7B-Instruct & 0.127 & $2.3 \times 10^{-135}$ \\
\bottomrule
\end{tabular}
}
\caption{Correlation between relevance scores (mean top-5) and downstream answer performance (Recall@3-gram) under different rerankers and generators.}
\label{tab:rerank_corr}
\vspace{-15pt}
\end{table}

==> tables/pearson_all.tex <==
\begin{table}[t]
\centering
\small
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|cc|cc}
\toprule
& \multicolumn{2}{c|}{\textbf{MKQA}} & \multicolumn{2}{c}{\textbf{XOR TyDi QA}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\textbf{Setting}
& \textbf{Pearson $r$} & \textbf{$p$-value}& \textbf{Pearson $r$} & \textbf{$p$-value}\\
\midrule
\multicolumn{5}{c}{\textbf{\textit{Command-R-35B}}} \\
\midrule
 BGE-Reranker   &0.198  & $<10^{-100}$ & 0.234  & $2.9\times10^{-40}$ \\ 
\quad\textbf{+ LAURA} &0.237  & $<10^{-100}$ & 0.174  & $1.3\times10^{-22}$ \\ 
Qwen-Reranker&0.158 & $<10^{-100}$ & 0.114 & $1.7\times10^{-10}$ \\ 
\quad\textbf{+ LAURA} & \textbf{0.287}  & $<10^{-100}$ & \textbf{0.304}  & $7.1\times10^{-68}$ \\ 

\midrule
\multicolumn{5}{c}{\textbf{\textit{Llama3-8B-Instruct}}} \\
\midrule
 BGE-Reranker   &0.198  & $<10^{-100}$ & 0.264  & $2.9\times10^{-40}$ \\ 
\quad\textbf{+ LAURA} &0.236  & $<10^{-100}$ & 0.184  & $3.5\times10^{-25}$ \\ 
Qwen-Reranker&0.157 & $<10^{-100}$ & 0.126 & $1.4\times10^{-13}$ \\ 
\quad\textbf{+ LAURA} & \textbf{0.274}  & $<10^{-100}$ & \textbf{0.327}  & $4.2\times10^{-79}$ \\ 

\midrule
\multicolumn{5}{c}{\textbf{\textit{Qwen2.5-7B-Instruct}}} \\
\midrule
BGE-Reranker   &0.188  & $<10^{-100}$ & 0.250  & $1.0\times10^{-45}$ \\ 
\quad\textbf{+ LAURA} &0.247  & $<10^{-100}$ & 0.192  & $1.9\times10^{-27}$ \\ 
Qwen-Reranker&0.161 & $<10^{-100}$ & 0.132 & $1.4\times10^{-12}$ \\ 
\quad\textbf{+ LAURA} &\textbf{0.292}  & $<10^{-100}$ & \textbf{0.311}  & $2.8\times10^{-71}$ \\ 

\bottomrule
\end{tabular}
}
\caption{Pearson correlation between reranker relevance scores (mean of top-5) and downstream answer performance (Recall@3-gram) on MKQA and XOR TyDi QA.}

\label{tab:rerank_corr_all}
\end{table}


==> tables/qa_res_train.tex <==
\begin{table}[t]
\centering
\small
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}[-0.8ex]{\textbf{Setting}} & \multicolumn{2}{c}{\textbf{Llama}} & \multicolumn{2}{c}{\textbf{Qwen}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & \textbf{3-gram} & \textbf{Pearson}& \textbf{3-gram} & \textbf{Pearson} \\
\midrule
    BGE-Reranker  &  48.9 &0.198 & 46.7 &0.188 \\
    \quad\textbf{+ LAURA} & \textbf{49.9} &\textbf{0.236} & \textbf{47.7} & \textbf{0.247}\\ 
    \midrule
    Qwen-Reranker  & 47.1&0.129 & 44.9&0.127 \\ 
    \quad\textbf{+ LAURA} & \textbf{49.2}& \textbf{0.269} & \textbf{46.7}& \textbf{0.264}\\ 
\bottomrule
\end{tabular}
}
\vspace{0pt}
\caption{Generation performance and Pearson correlation of rerankers before and after LAURA training on the MKQA test set. Pearson correlations are computed between the average reranker scores of the top-5 reranked documents and character 3-gram recall performance. All Pearson correlations are statistically significant with p-values < 0.001.}
\label{tab:qa_res_train}
\end{table}


